Specification and Implementation of Replicated List: The Jupiter Protocol Revisited

The replicated list object is frequently used to model the core functionality of replicated collaborative text editing systems. Since 1989, the convergence property has been a common specification of a replicated list object. Recently, Attiya et al. proposed the strong/weak list specification and conjectured that the well-known Jupiter protocol satisfies the weak list specification. The major obstacle to proving this conjecture is the mismatch between the global property on all replica states prescribed by the specification and the local view each replica maintains in Jupiter using data structures like 1D buffer or 2D state space. To address this issue, we propose CJupiter (Compact Jupiter) based on a novel data structure called $n$-ary ordered state space for a replicated client/server system with $n$ clients. At a high level, CJupiter maintains only a single $n$-ary ordered state space which encompasses exactly all states of each replica. We prove that CJupiter and Jupiter are equivalent and that CJupiter satisfies the weak list specification, thus solving the conjecture above.

==> sections/acknowledgment.tex <==
This work is supported by the National 973 Program of China (No. 2015CB352202),
the National Natural Science Foundation of China (No. 61702253),
and the Fundamental Research Funds for the Central Universities (No. 020214380031).


==> sections/authors.tex <==
% biography section
%
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}{Hengfeng Wei}
	Biography text here.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiographynophoto}{Yu Huang}
	Biography text here.
\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with biographies
%\newpage

\begin{IEEEbiographynophoto}{Jian Lu}
	Biography text here.
\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}



==> sections/cjupiter-property.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Properties of \cjupiter}  \label{ss:cjupiter-property}

By \textsc{xForm}, the edges labeled with the operations with the same $oid$ are ``parallel''
(Figure~\ref{fig:xform-ot}). 
Therefore,

%%%%%%%%%%%%%%% lemma:simple-path %%%%%%%%%%%%%%%
\begin{lemma}[Simple Path]  \label{lemma:simple-path}
  Let $P_{v_1 \leadsto v_2}$ be a path 
  from vertex $v_1$ to vertex $v_2$ in an $n$-ary ordered state space.
  Then, there are no duplicate operations (in terms of their $oid$s)
  along the path $P_{v_1 \leadsto v_2}$.
  We call such a path a simple path.
\end{lemma}
%%%%%%%%%%%%%%% lemma:simple-path %%%%%%%%%%%%%%%

The operation sequence with which an operation transforms \emph{at the server}
can be characterized as follows. 

%%%%%%%%%%%%%%% lemma:cjupiter-ot-server %%%%%%%%%%%%%%%
\begin{lemma}[\cjupiter{} OT Sequence] \label{lemma:cjupiter-ot-server}
  In \emph{\textsc{xForm}} of \emph{\cjupiter{}}, 
  the operation sequence $L$ (may be empty) with which an operation $op$ transforms at the server
  consists of the operations that are both totally ordered by `$\prec_{s}$' before 
  and concurrent by \emph{`$\parallel$'} with $op$.
  Furthermore, the operations in $L$ are totally ordered by `$\prec_{s}$'.
\end{lemma}
%%%%%%%%%%%%%%% lemma:cjupiter-ot-server %%%%%%%%%%%%%%%


==> sections/compatible-paths-proof.tex <==
% file: sections/compatible-paths-proof.tex

\begin{proof}
  We prove a stronger statement that
  \emph{each pair of vertices consisting of one vertex in $P_{v_0 \leadsto v_1}$
  and the other in $P_{v_0 \leadsto v_2}$ are compatible},
  by mathematical induction on the length $l$ of the path \pathplain{v_0}{v_2}.
  To this end, we first claim that

  \begin{claim}[One-step Compatibility]
    Suppose that vertices $v$ and $v'$ are compatible.
    Let $v''$ be the next vertex of $v'$ along the edge labeled with operation $o$
    which does not correspond to any element of the list in vertex $v$.
    Then, $v$ and $v''$ are compatible.
  \end{claim}
  
  \emph{Base Case.} $l = 0$. \pathplain{v_0}{v_2} contains only the vertex $v_0$.
  We shall prove that $v_0$ is compatible with every vertex along \pathplain{v_0}{v_1}.
  This can be done by mathematical induction on the length of \pathplain{v_0}{v_1}
  with the claim above and the fact that \pathplain{v_0}{v_1} is a simple path.
  
  \emph{Inductive Hypothesis.} Suppose that this lemma holds
  when the length of \pathplain{v_0}{v_2} is $l \geq 1$.
  
  \emph{Inductive Step.} We shall prove that the $(l+1)$-\emph{st} vertex, denoted $v_{l+1}$,
  of \pathplain{v_0}{v_2} is compatible with every vertex along \pathplain{v_0}{v_1}.
  This can be done by mathematical induction on the length of \pathplain{v_0}{v_1}
  with the claim above, the fact that \pathplain{v_0}{v_2} is a simple path (for $v_0$ and $v_{l+1}$ being compatible),
  and the fact that \pathplain{v_0}{v_1} and \pathplain{v_0}{v_2} are disjoint.
\end{proof}


==> sections/context-ot.tex <==
%%%%%%%%%%%%%%%%%%%% ss:context-ot %%%%%%%%%%%%%%%%%%%%
% \subsubsection{Context-based Operational Transformation} \label{sss:context-ot}

CP1 for $OT(o_1, o_2)$ requires that $o_1$ and $o_2$ be defined on the same state $\sigma$,
which is called the \emph{context} of them~\cite{Sun:TPDS09}.
In OT-based protocols, a replica state is often represented by the operations
the replica has processed.
Formally,

% There are two kinds of operations in an execution of an OT-based protocol:
% the original user operations and the transformed ones by OTs.
% Thus, the replica state defined in Definition~\ref{def:state} can be represented as follows.

%%%%%%%%%% def:state %%%%%%%%%%
\begin{definition}[Replica State Representation: Definition~\ref{def:replica-behavior} Revisited]   \label{def:re-state}
	Let $\alpha$ be a well-formed execution.
	A \emph{replica state} $\sigma$ of replica $R$
	is represented by the operations it has processed.
	% prefix subsequence of operations of $\alpha|_{R} \triangleq \seq{e_1, e_2, \ldots}$ it has processed.
	Specifically,
	\begin{itemize}
		\item The initial state is $\sigma_0 = \emptyset$; and
		\item After processing the $(i+1)$-\emph{st} operation $o_{i+1}$, the new replica state is
			$\sigma_{i+1} = \sigma_{i} \cup \set{\org{o_{i+1}}}$~\footnote{We use the set-theoretic notations here,
			because the ordering of the operations in $\sigma$ does not matter.},
			where $\org{o}$ denotes the original form of $o$.
	\end{itemize}
\end{definition}
%%%%%%%%%% def:state %%%%%%%%%%

Each operation is associated with a context
which determines with which and how it is transformed.

%%%%%%%%%% def:context %%%%%%%%%%
\begin{definition}[Operation Context]   \label{def:context}
	Let $\alpha$ be an execution.
	The \emph{context} of an operation $o$ in $\alpha$, denoted $C(o)$,
	is the replica state on which $o$ is defined:
	\begin{enumerate}
		\item for an original operation $o$, $C(o) = \sigma$,
			where $\sigma$ is the replica state from which $o$ is generated;
		\item for a transformed operation $o' = OT(o, o_x)$,
			$C(o') = C(o) \cup \set{\org{o_x}}$.
	\end{enumerate}
\end{definition}
%%%%%%%%%% def:context %%%%%%%%%%

Following~\cite{Xu:CSCW14}, we denote by \cop{o_1}{o_2} that $o_2$ is in the context of $o_1$.
Thus, the OT of transforming $o_1$ with $o_2$ can also be written as
$\copinmath{o_1}{o_2} = OT(o_1, o_2)$.

%%%%%%%%%% remark:org %%%%%%%%%%
\begin{remark}  \label{remark:org}
	By definition, operations in a context are all original ones.
	Causal and total ordering relations are also defined on original operations.
	For convenience, we assume an automatic conversion from $o$ to $\org{o}$,
	whenever necessary.
\end{remark}
%%%%%%%%%% remark:org %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% ss:context-ot %%%%%%%%%%%%%%%%%%%%


==> sections/css-op.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Operation}   \label{ss:css-op}

\begin{definition}[Operation]	\label{def:css-op}
  Each operation $op$ of type $\Op$ (Algorithm~\ref{alg:css-op}) consists of
  \begin{itemize}
    \item $o:$ the signature of type $\opset$ described in Section~\ref{ss:list-spec};
    \item $oid:$ a globally unique identifier,
      each of which is a pair $(rid, seq) \in \mathbb{N}_{0} \times \mathbb{N}_{0}$ 
      consisting of replica id and sequence number; 
    \item $ctx:$ an \emph{operation context} which is a set of operation identifiers,
      denoting the operations that have been executed before $op$; \emph{and}
    \item $sctx:$ the \emph{operation context at the server side}
      which is a set of operation identifiers,
      denoting the operations that have been executed before $op$ at server.
      We have that $op \so op'$ if and only if $op.oid \in op'.sctx$.
  \end{itemize}
\end{definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/disjoint-paths-proof.tex <==
% file: sections/disjoint-paths-proof.tex

%%%%%%%%%% fig:disjoint-paths-ladder %%%%%%%%%%
\begin{figure}[!t]
  \centering
  \begin{subfigure}[b]{0.38\textwidth}
    \includegraphics[width = \textwidth]{figs/disjoint-paths-extension-ladder.pdf}
    \caption{\textsc{Case 2.1:} $v_{\alpha} \xrightarrow{o} v'_{\alpha}$
    and $v_{\beta} \xrightarrow{o} v'_{\beta}$ are in the same ``extension ladder''.}
    \label{fig:disjoint-paths-extension-ladder}
  \end{subfigure}\hfil
  \begin{subfigure}[b]{0.52\textwidth}
    \includegraphics[width = \textwidth]{figs/disjoint-paths-step-ladder.pdf}
    \caption{\textsc{Case 2.2:} $v_{\alpha} \xrightarrow{o} v'_{\alpha}$
    and $v_{\beta} \xrightarrow{o} v'_{\beta}$ are in a ``step ladder''.}
    \label{fig:disjoint-paths-step-ladder}
  \end{subfigure}
  \caption{Illustrations of \textsc{Case} 2 of the proof for Lemma~\ref{lemma:disjoint-paths}:
    $v_1$ and $v_2$ are not in the same path from $v_0 = \text{LCA}(v_1, v_2)$.}
  \label{fig:disjoint-paths-ladder}
\end{figure}
%%%%%%%%%% fig:disjoint-paths-ladder %%%%%%%%%%

\begin{proof}
  We consider whether $v_1$ and $v_2$ are in the same path 
  from $v_0 = \text{LCA}(v_1, v_2)$ or not.
  
  \textsc{Case} \emph{1: $v_1$ and $v_2$ are in the same path from $v_0 = \emph{LCA}(v_1, v_2)$.}
  In this case, $v_0 = v_1$ or $v_0 = v_2$.
  Therefore, either $O_{v_0 \leadsto v_1}$ or $O_{v_0 \leadsto v_2}$ is empty.
  This lemma obviously holds. 
  
  \textsc{Case} \emph{2: $v_1$ and $v_2$ are not in the same path from $v_0 = \emph{LCA}(v_1, v_2)$.}
  In this case, we prove this lemma by contradiction.
  Suppose that
  % \begin{equation*}
  $o \in O_{v_0 \leadsto v_1} \cap O_{v_0 \leadsto v_2}$,
  % \end{equation*}
  where $o$ can be either original or transformed (identified by its $oid$).
  As illustrated in Figure~\ref{fig:disjoint-paths-ladder},
  the paths \pathplain{v_0}{v_1} and \pathplain{v_0}{v_2} are: 
  % \begin{align*}
  $\pathinmath{v_0}{v_1} = P_{v_0 \leadsto v_{\alpha} \xrightarrow{o} v'_{\alpha} \leadsto v_1}$
  and $\pathinmath{v_0}{v_2} = P_{v_0 \leadsto v_{\beta} \xrightarrow{o} v'_{\beta} \leadsto v_2}$.
  % \end{align*}
  In the following, we derive a contradiction that $v_0$ is not the unique LCA of $v_1$ and $v_2$.
  We consider two cases according to how the edges $v_{\alpha} \xrightarrow{o} v'_{\alpha}$
  and $v_{\beta} \xrightarrow{o} v'_{\beta}$ are related via OTs in \csss{}.
  
  \textsc{Case} \emph{2.1: $v_{\alpha} \xrightarrow{o} v'_{\alpha}$ and $v_{\beta} \xrightarrow{o} v'_{\beta}$ are
  in the same ``extension ladder'' structure of OTs.}
  Without loss of generality, we assume that $v'_{\beta}$ is reachable from $v'_{\alpha}$;
  as illustrated in Figure~\ref{fig:disjoint-paths-extension-ladder}.
  In this case, $v'_{\alpha}$ is a \emph{lower} common ancestor of $v_1$ and $v_2$ than $v_0$.
  
  \textsc{Case} \emph{2.2: $v_{\alpha} \xrightarrow{o} v'_{\alpha}$ and $v_{\beta} \xrightarrow{o} v'_{\beta}$ are
  in a ``step ladder'' structure of OTs.}
  Because all the edges labeled with the same operation $o$ are constructed directly or indirectly
  from the OTs involving the original form of $o$,
  there exists some edge $v_{\gamma} \xrightarrow{o} v'_{\gamma}$ that is in the same ``extension ladder''
  with $v_{\alpha} \xrightarrow{o} v'_{\alpha}$ as well as with $v_{\beta} \xrightarrow{o} v'_{\beta}$;
  as illustrated in Figure~\ref{fig:disjoint-paths-step-ladder}.
  In this case, $v'_{\gamma}$ is a common ancestor of $v_1$ and $v_2$ \emph{other than} $v_0$.
\end{proof}


==> sections/dist-jupiter.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Distributed \jupiter{} Protocol}  \label{section:djupiter}

% By orthogonally integrating the $n$-ary ordered state space
% with a distributed scheme to totally order operations,
% we further extend \cjupiter{} to a distributed setting.

Recall that the construction of $n$-ary ordered state space at each replica is
determined by the schedule of operations,
namely the causal and total orderings on operations.
Being distributed, the \djupiter{} (Distributed \jupiter{}) protocol
relies on an atomic broadcast~\cite{Defago:CSUR04, Attiya:Book04} to totally order operations.
% Taking into account the requirement of preserving causality,
Specifically, \djupiter{} assumes a causal atomic broadcast service~\cite{Attiya:Book04, Attiya:PODC16}
and behaves as \cjupiter{} with two exceptions:
%%%%%%%%%% the DCSS protocol %%%%%%%%%%
\begin{enumerate}
  \item In the case of a replica generating an operation $o$,
    the replica finally broadcasts $o$ to all replicas (including itself),
    utilizing the causal atomic broadcast service.
  \item Each replica receives and processes operations in the order
    enforced by the causal atomic broadcast service,
    ignoring the operations it generates.
\end{enumerate}
%%%%%%%%%% the DCSS protocol %%%%%%%%%%

\djupiter{} is a \emph{simulation} of \cjupiter{},
by replacing the central server in \cjupiter{} with an atomic broadcast service.
Thus, it also satisfies the weak list specification $\wlspec{}$.

%%%%%%%%%% prop:simulation %%%%%%%%%%
\begin{prop}[Simulation]    \label{prop:simulation}
  Let $\protinmath = \set{R_1, \ldots, R_n, S}$ be the \emph{\cjupiter{}} protocol
  running on a client/server system with $n$ clients $R_1, \ldots, R_n$ and a server $S$.
  Let $\protinmath' = \set{R'_1, \ldots, R'_n}$ be the \emph{\djupiter{}} protocol
  running on a distributed system with $n$ replicas.
  Then $\protinmath'$ is a simulation of \prot{} in the sense that
  for any execution $\alpha'$ of $\protinmath'$,
  there exists an execution $\alpha$ of \prot{} such that
  $\alpha|_{R_i}^{\doe} = \alpha'|_{R'_i}^{\doe}\, , 1 \leq i \leq n$.
  % \begin{equation*}
  %   \alpha|_{R_i}^{\doe} = \alpha'|_{R'_i}^{\doe}\, , \quad 1 \leq i \leq n.
  % \end{equation*}
\end{prop}
%%%%%%%%%% prop:simulation %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/irreflexivity-proof.tex <==
% file: sections/irreflexivity-proof.tex

%%%%%%%%%%%%%%% proof:irreflexivity %%%%%%%%%%%%%%%
\begin{proof} \textbf{(For Lemma~\ref{lemma:irreflexivity}.)}
  ``$\Longleftarrow$'' \emph{(if):}
  Suppose by contradiction that $\lorel{a}{a}$ for some $a \in \elems{H}$.
  According to Lemma~\ref{lemma:simple-path}, a list state $w$ contains no duplicate elements.
  Therefore, there exist two list states such that for some element $b$,
  $\lorel{a}{b}$ (namely, $a$ precedes $b$) in one state
  and $\lorel{b}{a}$ (namely, $b$ precedes $a$) in the other.
  However, this contradicts the assumption that all list states are pairwise compatible.
  
  ``$\implies$'' \emph{(only if):}
  Suppose by contradiction that two list states $w_1$ and $w_2$ are incompatible.
  That is, they have two common elements $a$ and $b$ such that
  $a$ precedes $b$ in, say, $w_1$ and $b$ precedes $a$ in $w_2$.
  Thus, both $\lorel{a}{b}$ and $\lorel{b}{a}$ hold.
  Since \lo{} is transitive on $w_1$ (and $w_2$), we have $\lorel{a}{a}$,
  contradicting the assumption that \lo{} is irreflexive.
\end{proof}
%%%%%%%%%%%%%%% proof:irreflexivity %%%%%%%%%%%%%%%



==> sections/jupiter-sched-behavior.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{A Framework for OT-based Protocols}    \label{sss:jupiter-framework}

Jupiter adopts a centralized client/server architecture.
Collaborating clients are connected to a central server via TCP connections.
All communication channels, from clients to the server or in the other direction, are FIFO.
For convenience, we assume that the server does not
generate operations~\cite{Xu:CSCW14, Attiya:PODC16}.
It mainly serializes operations and propagates them from one client to others.

This work contains two Jupiter protocols.
Section~\ref{section:cscw-protocol} reviews the existing Jupiter protocol
described in the CSCW paper~\cite{Xu:CSCW14} that we call the CSCW Jupiter protocol.
Section~\ref{section:css-protocol} proposes a new Jupiter protocol called the CSS Jupiter protocol.
% Though \grammar{differing in the way of \emph{processing} operations at replicas},
% they follow the same communication pattern: \todo{cont.}
To facilitate the comparison of these two protocols later on,
we describe them in a uniform framework which separates the \emph{schedule} of messages/operations
from replica behaviors (Definition~\ref{def:replica-behavior})
in an execution of a protocol.
A schedule is concerned with only the temporal aspect of an execution.
Formally,

%%%%%%%%%% def:sched %%%%%%%%%%
\begin{definition}[Schedule]   \label{def:sched}
	Let $\alpha$ be an execution.
	The \emph{schedule} of $\alpha$ is $\alpha$
	with the arguments of each event erased.
\end{definition}
%%%%%%%%%% def:sched %%%%%%%%%%

%%%%% fig:jupiter-schedule-c3o3 %%%%%
\begin{figure}[t]
	\centering
	\includegraphics[width = 0.32\textwidth]{figs/jupiter-schedule-c3o3.pdf}
	\caption{An schedule consisting of 3 pairwise concurrent operations.}
	\label{fig:jupiter-schedule-c3o3}
\end{figure}
%%%%% fig:jupiter-schedule-c3o3 %%%%%

A schedule is depicted as a ``space-time diagram'' such as Figure~\ref{fig:jupiter-schedule-c3o3}.
In both Jupiter protocols, we will see that
it is the causal and total orderings (Definitions~\ref{def:causal} and \ref{def:total}) on user operations
in a schedule that determine which OTs are performed and in what order,
which in turn, together with the OT functions, determine the behavior of each replica.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/jupiter-strong-spec.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Jupiter Violates the Strong List Specification}  \label{ss:jupiter-strong-spec}

%%%%%%%%%% thm:sl-spec %%%%%%%%%%
\begin{theorem}[$\css{} \not\models \slspec{}$]   \label{thm:sl-spec}
	The \css{} protocol (or equivalently, the \cscw{} protocol)
	does not satisfy the strong list specification $\slspec{}$ (Definition~\ref{def:sl-spec}).
\end{theorem}

%%%%% fig:jupiter-not-strong %%%%%
% fig:jupiter-schedule-podc16
% fig:jupiter-css-podc16
\begin{figure}[!t]
	\centering
	\begin{subfigure}[b]{0.35\textwidth}
		\includegraphics[width = \textwidth]{figs/jupiter-schedule-podc16.pdf}
		\caption{A schedule adapted from Figure~1 of~\cite{Attiya:PODC16}.}
		\label{fig:jupiter-schedule-podc16}
	\end{subfigure}
	
	\begin{subfigure}[b]{0.40\textwidth}
		\includegraphics[width = \textwidth]{figs/jupiter-css-c3o4-podc16.pdf}
		\caption{The $n$-ary ordered state-space produced by the \css{} protocol.
		As illustrated, the server and client $c_1$ go along the path $0 \to 1 \to 12 \to 123 \to 1234$,
		client $c_2$ goes along the path $0 \to 1 \to 13 \to 123 \to 1234$,
		and client $c_3$ goes along the path $0 \to 1 \to 14 \to 124 \to 1234$.
		(We assume that client with a larger id has a higher priority.)}
		\label{fig:jupiter-css-podc16}
	\end{subfigure}
	\caption{A counterexample showing that Jupiter does not satisfy the strong list specification.}
	\label{fig:jupiter-not-strong}
\end{figure}
%%%%% fig:jupiter-not-strong %%%%%

\begin{proof}
	Figure~\ref{fig:jupiter-not-strong} shows a counterexample,
	including a schedule adapted from Figure~1 of~\cite{Attiya:PODC16}
	and the $n$-ary ordered state-space produced by the \css{} protocol.
	Initially, the replicated list is empty, namely $w = \epsilon$.
	The fact that the strong list specification is not satisfied by this execution
	follows from:
	\begin{itemize}
		\item The list $w_{13}$ in state $\sigma_{13} = \set{1,3}$ of client $c_2$ is $ax$;
		\item The list $w_{14}$ in state $\sigma_{14} = \set{1,4}$ of client $c_3$ is $xb$;
		\item The list $w_{1234}$ in the same final state $\sigma_{1234} = \set{1,2,3,4}$ of all replicas is $ba$;
		\item According to condition 1) of the strong list specification,
			the list order \lo{} would have to be
			\begin{equation*}
				\lo{} = \set{(a,x), (x,b), (b,a)};
			\end{equation*}
		\item However, the list order \lo{} above contains a cycle,
			contradicting condition 2) of the strong list specification.
	\end{itemize}
\end{proof}
%%%%%%%%%% thm:sl-spec %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/keywords.tex <==
\keywords{
Collaborative text editing,
Replicated list,
% Concurrency control,
Convergence,
Strong/weak list specification,
Operational transformation,
Jupiter.
}


==> sections/ordering.tex <==
%%%%%%%%%%%%%%%%%%%% ss:ordering %%%%%%%%%%%%%%%%%%%%
% \subsubsection{Orderings on User Operations and Schedule}   \label{sss:ordering}

% Let $\alpha$ be an execution and $A = (H, \vis{})$ an abstract execution
% such that $H$ is the subsequence of all $\doe{}$ events
% (corresponding to user operations) in $\alpha$.

OT-based protocols rely on causal relation on user operations
to determine which operations should be transformed with which others.

\begin{comment}
%%%%%%%%%% def:causal %%%%%%%%%%
\begin{definition}[Causal Relation `$\causal$'] \label{def:causal}
	Event $e \in H$ is \emph{causally before} event $e' \in H$,
	denoted $\crel{H}{e}{e'}$ (or $\crel{}{e}{e'}$),
	if and only if $\hbrel{\alpha}{e}{e'}$ in $\alpha$.
\end{definition}
%%%%%%%%%% def:causal %%%%%%%%%%

%%%%%%%%%% def:concurrent %%%%%%%%%%
\begin{definition}[Concurrent Relation `$\parallel$']   % \label{def:concurrent}
	Events $e, e' \in H$ are \emph{concurrent},
	denoted $\pararel{H}{e}{e'}$ (or $\pararel{}{e}{e'}$),
	if and only if neither $\crel{H}{e}{e'}$ nor $\crel{H}{e'}{e}$.
\end{definition}
%%%%%%%%%% def:concurrent %%%%%%%%%%

TOOT-based protocols further rely on a total ordering relation on user operations,
that is consistent with the causal relation,
% that is consistent with the causal ordering on the same group of operations
to control the transformation orders~\cite{Xu:CSCW14}.

%%%%%%%%%% def:total %%%%%%%%%%
\begin{definition}[Total Ordering Relation `$\total$'] % Consistent with Causal Relation `$\causal$`]
	\label{def:total}
	Event $e \in H$ is before event $e' \in H$ in the \emph{total ordering relation} `$\total$',
	denoted $\trel{H}{e}{e'}$ (or $\trel{}{e}{e'}$),
	if and only if $\tbrel{\alpha}{e}{e'}$.
\end{definition}
%%%%%%%%%% def:total %%%%%%%%%%
\end{comment}

To emphasize the orderings on operations,
we separate the \emph{schedule} of operations from replica behaviors
in an execution of a protocol.
Intuitively, a schedule is concerned with only the temporal aspect of an execution,
depicted as a ``space-time diagram'' such as Figure~\ref{fig:jupiter-schedule-c3o3}.
More precisely,

%%%%%%%%%% def:sched %%%%%%%%%%
\begin{definition}[Schedule]   \label{def:sched}
Let $\alpha$ be an execution.
The \emph{schedule} of $\alpha$ is $\alpha$
with the arguments of each event erased.
\end{definition}
%%%%%%%%%% def:sched %%%%%%%%%%

\begin{ppopp18figure}
%%%%% fig:jupiter-schedule-c3o3 %%%%%
\begin{figure}[t]
	\centering
	\includegraphics[width = 0.26\textwidth]{figs/jupiter-schedule-c3o3.pdf}
	\caption{A schedule consisting of three pairwise concurrent operations.}
	\label{fig:jupiter-schedule-c3o3}
\end{figure}
%%%%% fig:jupiter-schedule-c3o3 %%%%%
\end{ppopp18figure}

% A schedule is depicted as a ``space-time diagram'' such as Figure~\ref{fig:jupiter-schedule-c3o3}.
% We compare protocols under the same schedule.
%%%%%%%%%%%%%%%%%%%% ss:ordering %%%%%%%%%%%%%%%%%%%%


==> sections/preliminary-jupiter.tex <==
% file: preliminary-jupiter.tex

The CSCW Jupiter protocol~\cite{Xu:CSCW14}
is a complete \emph{multi-client} description of Jupiter
first proposed in~\cite{Nichols:UIST95}.
It adopts a centralized client/server architecture.
Clients are connected to a central server via FIFO channels.
For convenience, we assume that the server does not
generate operations~\cite{Xu:CSCW14, Attiya:PODC16}.
It mainly serializes operations and propagates them from one client to others.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Data Structure: 2D State-spaces}    \label{sss:cscw-2d}
%
Suppose that the client/server system includes $n$ clients.
CSCW maintains $2n (= n + n)$ \emph{2D state-spaces},
each of which consists of a \emph{local} dimension and a \emph{global} dimension.
Each client $c_i$ maintains a state-space, denoted \cscwc{i},
with the local dimension for operations generated by the client
and the global dimension for operations generated by other clients.
The server maintains $n$ 2D state-spaces, one for each client.
The state-space for client $c_i$, denoted \cscws{i},
consists of the local dimension for operations from client $c_i$
and the global dimension for operations from other clients.


==> sections/preliminary-ot-jupiter.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{OT: Operational Transformation} \label{ss:preliminary-ot-jupiter}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \input{sections/ordering}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{sections/preliminary-ot}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \input{sections/preliminary-jupiter}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \input{sections/context-ot}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \input{sections/jupiter-sched-behavior}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> sections/weak-vs-ec.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Weak List Specification \emph{vs.} Convergence Property}	\label{ss:weak-vs-cp}

Q: Weak list specification $\implies$ convergence property?

A: Yes! Proved by~\cite{Attiya:PODC16}.

Q: Convergence property $\implies$ weak list specification?

A: \question{???} Find protocols ensuring the convergence property but not weak list specification?

Q: {Identify separate algorithmic mechanisms for weak list specification and convergence property.}

A: Do not know yet.

Q: Role of the ``Leftmost'' property in the CSS protocol?

A: Lattice construction???
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

